On the Smoothness and Regularity of the Chess Billiard Flow and the Poincar\'e Problem

The Poincar\'e problem is a model of two-dimensional internal waves in stable-stratified fluid. The chess billiard flow, a variation of a typical billiard flow, drives the formation behind and describes the evolution of these internal waves, and its trajectories can be represented as rotations around the boundary of a given domain. We find that for sufficiently irrational rotation in the square, or when the rotation number $r(\lambda)$ is Diophantine, the regularity of the solution $u(t)$ of the evolution problem correlates directly to the regularity of the forcing function $f(x)$. Additionally, we show that when $f$ is smooth, then $u$ is also smooth. These results extend studies that have examined singularity points, or the lack of regularity, in rational rotations of the chess billiard flow. We also present numerical simulations in various geometries that analyze plateau formation and fractal dimension in $r(\lambda)$ and conjecture an extension of our results. Our results can be applied in modeling two dimensional oceanic waves, and they also relate the classical quantum correspondence to fluid study.

==> appa.tex <==
% This is appa.tex
%
% This file is for appendices.  If you don't have any appendices, delete
% the percent sign from the beginning of the next line.
%\endinput

\appendix
\gdef\thesection{Appendix \Alph{section}}
% Add additional appendices by replicating the line below.

%\section{Title of Appendix}  

%Appendices may appear after the paper proper.  Appendices may hold
%extra information that would interrupt the flow of the paper and that
%is not absolutely necessary for the reader to appreciate the work.
%For example, a large number of related figures or a mathematical
%derivation could go nicely in an appendix.

\appendix

\section{Appendix Title}

This is a good place to put code, raw data, extra figures, etc.


==> summary.tex <==
% This is summary.tex

\noindent Internal waves, which help map the movement of a fluid, are important to the study of oceanography. These waves can be described and studied by mathematical equations, such as the Poincaré problem, which is one model of waves in two dimensions. We study this problem and its relation to a geometric map resembling pool billiard trajectories, where trajectories form by bouncing and reflecting off of the boundary of the shape. We show that given some particular parameters in the Poincaré problem, the evolution of the waves eventually becomes very smooth. The ocean can be very difficult to model, so studying changes in such two dimensional wave models can help analyze them. 
